SPIN: Sparsifying and Integrating Internal Neurons in Large Language Models for Text Classification

Among the many tasks that Large Language Models (LLMs) have revolutionized is text classification. Current text classification paradigms, however, rely solely on the output of the final layer in the LLM, with the rich information contained in internal neurons largely untapped. In this study, we present SPIN: a model-agnostic framework that sparsifies and integrates internal neurons of intermediate layers of LLMs for text classification. Specifically, SPIN sparsifies internal neurons by linear probing-based salient neuron selection layer by layer, avoiding noise from unrelated neurons and ensuring efficiency. The cross-layer salient neurons are then integrated to serve as multi-layered features for the classification head. Extensive experimental results show our proposed SPIN significantly improves text classification accuracy, efficiency, and interpretability.

==> tex/preliminary.tex <==
\section{Preliminaries}

The foundational structures of transformer-based language models comprise three principal components: (1) an \emph{embedding} module at the beginning, focusing on the translation of input token sequence with length $N$ to dense vector $\bm{X}_0\in\mathbb{R}^{N\times D}$ in the high-dimensional embedding space, (2) $L$ identical \emph{encoder} or \emph{decoder blocks}, each of which contains a multi-head attention module and a feed-forward network (FFN) jointly applying nonlinear transformations $\bm{X}_l \mapsto \bm{X}_{l+1}$, and (3) a \emph{model head} on top of the last-layer hidden states that reshapes and refines representation outputs to generate the desired final output.

Conventionally, the last-layer hidden states $\bm{X}_L$ are condensed in a token-wise manner at sentence level by picking the values at the specific position, e.g. \verb+[CLS]+ at the beginning of each sentence in BERT or the last token of each sentence in GPT family. \rmv{The comprehensive information of the sentence is gathered at a single token typically due to the variance of sentence length.}The condensed sentence information is then either subsequently passed to language model head
to output the predicted probability distribution of next token, or to the classification head to output the label of the input text.
%a linear layer followed by a softmax activation to output the probability distribution of next token predicted as the language model head, or passed to several layers to output the label of input text as the classification head. 

\rmv{$g(\bm{X}_L,f_\text{single}:\mathbb{R}^N\mapsto\mathbb{R}): \mathbb{R}^{N\times D} \mapsto \mathbb{R}^D$}

==> tex/rmv.tex <==
\rmv{
\paragraph{Layer-wise Probing}
\label{lr}
The classification performance of layer-wise linear probes is regarded as an important indicator for measuring the knowledge acquisition in individual layers. To maintain a non-overfitting evaluation of the best per-layer performance, however, it is crucial to note that we treat both the pooling function and the layer \emph{l} as hyper-parameters. Meanwhile, as the best number of iterations for training the probes cannot be determined in advance, we also treat it as a hyper-parameter with a sufficient maximum limit. 

Consequently, the test performance we report is derived from applying this best combination of hyper-parameters, as determined by the validation set, ensuring that our reported results are not overfitted. Our findings are presented in the \textbf{Probes} column of Table \ref{tab:best_compare}, demonstrating the fact that the best individual layer performance of both frozen and fine-tuned models could be close to, and mostly even well above the results using their respective classification heads. 

In addition, to corroborate the linear representation hypothesis in our selected models and datasets, we also examine the more expressive nonlinear single layer perceptrons (SLP) probes as the comparative group to LR probes. We report the details and results of SLP in \ref{SLP}.
}

\paragraph{Feature Sparsification} \rmv{In the first stage, at each layer of the LLM, a linear probe with $\mathcal{L}^1$-regularization is applied to the activations and hidden states. This process is aimed at identifying the most salient neurons in the layer, which are most predictive of the output categories. The LR model is trained to minimize the sum of the $\mathcal{L}^1$-norm of the weights and the error in predicting the output categories, which facilitates the selection of the most relevant features while penalizing less important ones.} 

For each layer of the model, we firstly train a Lasso regressor as probe for each pooling choice of the internal representations. The number of iterations to train the probe and the coefficient of $\mathcal{L}^1$-regularization are treated as hyperparameters and optimized by the validation set. 

\rmv{In addition, to corroborate the linear representation hypothesis in our selected models and datasets, we also examine the more expressive nonlinear single layer perceptrons (SLP) probes as the comparative group to our LR probes. We report the details and results of best layer-wise probes in \emph{Appendix}.} 

\textcolor{blue}{TODO: This part should somehow go to Methodology}

Once the layer-wise probes are fitted, the weights of the linear models are sorted in descending order, after which the most indicative neurons on the specific task are selected based on their contribution to the model's predictive power. This selection procedure is achieved by accumulating the squared weights of the neurons until a predefined sparsification threshold, $\eta$, of the total squared weight magnitude is reached. The neurons that meet this criterion are then marked as salient for the corresponding layer and prepared for further aggregation. In practice, we have $\eta$ ranged from 0.001 to 0.5, indicating a wide range of levels in sparsification with the number of neurons selected per layer ranging from 1 to around 5\%-10\% of total. 

\textcolor{blue}{TODO: We need some figs to corroborate this}

Our sparsification results confirm the findings of \citet{wang2022finding} and \citet{gurnee2023finding} where a minimal amount of most informative neurons could embrace comparable performance with the model classification head, yet within single layer and without further aggregation, we have not found evidence that using only sparsified neurons could yield better performance than than the entire layer-wise probes.\rmv{\footnote{Intuitively, as $\eta$ increases with more relevant neurons selected, the classification performance of the selected neurons tend to be more stable and closer to the layer-wise probes if the probes are well-trained.} Thus, to visually demonstrate how well feature sparsification actually works, we refer to Section \ref{interp} with further details showcasing the intrinsic interpretability of STC's sparsification process.} 


\xhdr{Multi-layer Aggregation} 
Finally, the salient neurons identified across different layers of the LLM are combined to form an aggregated representation. This representation is then used to train a new LR model, which is called \emph{then-Classify} and aligns with our aforementioned linear representation hypothesis\footnote{Note that linear models may not and have to be not optimal for different cases. However, we present the linear model as a na\"ive and intuitive approach which is already sufficient to attain the consistent performance boost in various cases.}. The aggregated LR models, starting from the bottom layer and extending to each subsequent layers, are then evaluated based on their performance in predicting the output categories. 

\textcolor{blue}{Experiments needed to show the tradeoff for using larger $\eta$ and more layers to inference. cue the papers of early-exit. }

Similar to layer-wise sparsification, the predetermined parameters, such as the threshold $\eta$, the choices of pooling methods, and the number of layers to aggregate, are all regarded as hyperparameters and optimized with validation set. We report the results based on the test performance of the re-trained classifier that demonstrates the best performance on the validation set in the STC column of Table \ref{tab:performance-pretrained} and \ref{tab:performance-finetuned}. 

\rmv{
\begin{table}[t]
    \centering
    \small
    \begin{tabular}{@{\hspace{4pt}}l@{\hspace{4pt}}|@{\hspace{4pt}}c@{\hspace{6pt}}c@{\hspace{4pt}}|@{\hspace{4pt}}c@{\hspace{6pt}}c@{\hspace{4pt}}|@{\hspace{4pt}}c@{\hspace{6pt}}c@{\hspace{4pt}}}
    \toprule
         & \multicolumn{2}{@{\hspace{0pt}}c@{\hspace{4pt}}|@{\hspace{4pt}}}{\textbf{IMDb}} & \multicolumn{2}{@{\hspace{0pt}}c@{\hspace{4pt}}|@{\hspace{4pt}}}{\textbf{SST-2}} & \multicolumn{2}{@{\hspace{0pt}}c@{\hspace{4pt}}}{\textbf{EDOS}}  \\
        \cmidrule(l{-3pt}r){2-3} \cmidrule(l{-3pt}r){4-5} \cmidrule(l{-3pt}){6-7}
        \textbf{LLM} & m.o. & STC & m.o. & STC & m.o. & STC \\
    \midrule
        DistilBERT  & 86.95 & \textbf{89.49} & 84.06 & \textbf{84.40} & 65.09 & \textbf{75.79} \\
        RoBERTa     & 89.67 & \textbf{93.61} & 84.06 & \textbf{90.59} & 68.81 & \textbf{73.50} \\
        GPT2        & 87.72 & \textbf{91.94} & 85.89 & \textbf{87.73} & 68.57 & \textbf{76.08} \\
        GPT2-M      & 88.59 & \textbf{93.37} & 86.12 & \textbf{90.25} & 71.17 & \textbf{75.74} \\
        GPT2-L      & 91.75 & \textbf{94.36} & 90.14 & \textbf{91.97} & 72.05 & \textbf{76.33} \\
        GPT2-XL     & 91.86 & \textbf{94.92} & 90.02 & \textbf{93.23} & 72.56 & \textbf{76.79} \\
       % XLNet       & 86.42 & \textbf{93.15} & & & & \\
        Flan-T5-S   & 82.58 & \textbf{91.48} & 75.00 & \textbf{88.99} & 59.62 & \textbf{74.51} \\
        Flan-T5-M   & 89.26 & \textbf{94.15} & 85.89 & \textbf{92.32} & 66.64 & \textbf{78.04} \\
        Flan-T5-L   & 85.74 & \textbf{96.02} & 77.41 & \textbf{94.84} & 69.58 & \textbf{79.00} \\
        Flan-T5-XL  & 90.31 & \textbf{96.13} & 84.75 & \textbf{95.64} & 70.08 & \textbf{81.48} \\
    \midrule
        SoTA        & \multicolumn{2}{@{\hspace{0pt}}c@{\hspace{4pt}}|@{\hspace{4pt}}}{96.21} & \multicolumn{2}{@{\hspace{0pt}}c@{\hspace{4pt}}|@{\hspace{4pt}}}{97.50} & \multicolumn{2}{@{\hspace{0pt}}c@{\hspace{4pt}}}{82.35} \\
    \bottomrule
    \end{tabular}
    \caption{Experiment results of model output (m.o.) classification baseline and \emph{Sparsify-then-Classify} (STC) on frozen pretrained LLMs}
    \label{tab:performance-pretrained}
    \vspace{-0.2in}
\end{table}
}


For a given language model, we train and evaluate the classifier on aggregated features for each combination of pooling function, the number of aggregated layers, together with the sparsification threshold. We refer to Figure \ref{fig:www-gpt2xl} as \emph{what-which-where} plots. The \emph{what-which-where} plots visualize the performance regarding \emph{what} sparsification threshold is used, \emph{which} pooling choice is selected, and \emph{where} in depth the layer aggregation takes place in LLMs. Respectively, the pooling choice is indicated with different marker shapes, the magnitude of sparsification threshold is reflected by the marker sizes, and the number of aggregated layers is shown with different colors in the color bar. Additionally, we present how the number of total neurons selected during STC evolves with every combination of \emph{what-which-where} in the lower subfigures of each plot. \rmv{For a comprehensive list of what-which-where plot results in every specific case, please refer to \ref{www}.}

%\subsection{Understanding the Performance of STC}


%\subsection{STC and Supervised Fine-tuning}

%\textcolor{blue}{TODO: }
\subsubsection{STC on Fine-tuned LLM}

\paragraph{Internal Neurons Always Outperform Model Outputs.}
Our experimental evaluations yield a \textbf{consistent} improvement in performance by integrating our method into well-established transformer-based models with both pretrained and fine-tuned weights, since STC adopts a more granular approach by delving into the multi-layered architecture of transformer-based LLMs hidden beneath the final layer outputs. This verifies our previous testament about the confined informativeness by conventional classification methodologies' only using single tokens on the final layer output, and the robustness of our approach that rediscovers the capabilities of inner representation in capturing essential features.

\subsubsection{STC vs. SFT}
\paragraph{Pretrained Model Neurons Can Outperform Fine-tuned Models.}
Although our approach working on fine-tuned models still yields better performance than frozen pretrained ones, which fits the logic that fine-tuning has enhanced the salience of model inner representations in capturing task-specific features as well, a more intriguing pattern could be found that for larger models, internal neurons from pretrained models can already outperform previous SotA fine-tuned baselines. This suggests a relationship between the size of LLMs and their amenability to fine-tuning, that for larger LLMs, the less improvement SFT brings, since larger pretrained models already hold greater capacity for learning and generalization. Also, the increase in size makes the models harder to be effectively fine-tuned, as with their vast number of parameters, larger models can be more prone to overfitting when fine-tuned on small datasets. 

\paragraph{STC is More Efficient than SFT to Train }

\rmv{
\paragraph{Layer Aggregation Allows Compressing Model Sizes During Inference.}
As has already been illustrated in Figure \ref{fig:gpt2xl_lr_agg_compare}, the STC performance is mostly enhanced in the lower half of LLM layers, with only marginal improvements in the rest part of the model. This qualitative observation agrees with our initial idea of introducing layer aggregation as mentioned in \ref{cross-layer-aggregation} that the lower layers of LLMs are sufficiently salient for capturing task-specific features within input texts. Here we further compare the baseline performance of conventional classification heads with our STC method aggregating different proportions of the lower model layers to quantitatively substantiate the possibility of only running part of the LLM forward pass during inference. With our results in Table \ref{tab:inference_performance}, we can observe that for most cases, utilizing the first 60\% layers of the model is sufficient for STC to outperform the corresponding baselines that employ full model forward passes. In practice, after training and determining an optimal $L_\text{temp}$ that balances performance and efficiency as expected, our method can operate efficiently using only initial segments of LLMs, reducing both the storage needs for model weights and the computational time required for inference, particularly in efficiency-critical real-world application scenarios that are more speed- and resource-management-focused and less sensitive to performance metrics.

\paragraph{Multi-task Learning Can Further Amplify Efficiency.}
The approaches working on internal neurons do not modify model weights and hence are inherently suitable for a multi-task learning workflow. This stands in stark contrast to the model fine-tuning approach, which necessitates the training and independent storage of task-specific model weights for each task. Once the most compute-intensive acquisition of inner representations from input texts is complete, multiple salient feature sparsification and layer aggregation processes can not only proceed with their training phases respectively focusing on different features for specific tasks in perfect parallel, but are also allowed to generate results in inference at the same time with maintaining the same level of task-specific performance as if they were operating independently. Therefore, in cases where multiple tasks are present, our STC approach showcases a significant advantage over model fine-tuning by achieving multiple times savings in model weight storage as reported in Table \ref{tab:trainable-parameters} of trainable parameters and speedups in training floating point operation costs as in Table \ref{tab:training_cost}.
}

%\subsection{STC During Inference}
%\subsubsection{Efficiency from Early-exit}
%\subsubsection{Case Study: Interpretability at Application}
%\label{interp}
%transparency-demanding real-world applications
 



%\jt{maybe for next paper...}
%\paragraph{Knowledge consolidation}
%The inherent nature of the knowledge consolidation process allows better compatibility on %training sets. \jt{figures investigating using different proportions of training sets for layer-%independent salient neuron identification and knowledge consolidation across layers}


\rmv{Note that results matching HuggingFace model reports are marked with an asterisk, with a margin of error under 0.1\% validated. Unpublished model performances are based on our test results.}


\rmv{Within each transformer block in the models, the activations of the Feed-Forward Neural Network, which comprises $A=kD$ neurons in each transformer block, along with block hidden states comprising $D$ neurons in between transformer blocks, are collected, pooled, and stored.}

\rmv{
\paragraph{Inner Represetation Acquisition}

We replicated and validated the forward pass of 
DistilBERT, RoBERTa base, GPT2 base, GPT2-M, GPT2-L, GPT2-XL and Flan-T5 family to access their internal representations, integrating with both pretrained and fine-tuned weights sourced from HuggingFace\footnote{\url{https://huggingface.co/}}. Within each transformer block in the models, the activations of the Feed-Forward Neural Network, which comprises $A=kD$ neurons in each transformer block, along with block hidden states comprising $D$ neurons in between transformer blocks, are collected, pooled using $f \in\{f_\text{avg},f_\text{max},f_\text{single}\}$, and stored.
}

%\subsection{Model Output Performance}

\rmv{
For encoder-based models, they take the output of \verb+[CLS]+ token in the final hidden states for text classification. For decoder-based models, they take the final hidden states output of the last valid token for each input sequence on the other hand. Thus, We collect the output of the first \verb+[CLS]+ token in the last layer hidden states for BERT and its variants, and output of the last valid tokens for each sentence in the last layer hidden states from GPT2 and its variants. This criteria as well applies to Flan-T5 family where the lower half of the model is encoder-based and the upper half is decoder-based. 

Afterwards, a fully connected layer with softmax is then trained on top of the encoder or decoder output to determine the label of the input sentence.  Note that several models, especially fine-tuned ones, downloaded from HuggingFace have published their model output performance on certain datasets. For those models whose performance is publicly available, we adopt the official performance by marking them with an asterisk, and validate that the margin of error between our and their results is acceptable (normally within 0.1\%). For those models whose performance is unpublished, we use the test results in our experiments.
}

\rmv{ \textcolor{blue}{TODO: Maybe to Appendix.}
The precise feature ranking requires progressive multi-step filtering \citep{lecun1989optimal, dalvi2019one}. As another cross-layer aggregation structure would be trained above the filtered results, an accurate ordering of features in the phase of sparsification is unnecessary, hence our greedy layer-wise sparsification strategy simply approximates a 1-step backward elimination process and removes the least promising features efficiently. The probes adopt a perspective where seemingly irrelevant neurons can often provide a more comprehensive understanding in combination \citep{guyon2003introduction}, which enables our cross-layer aggregation process to further capture the nuances within sparsified features.
}

\rmv{
\textcolor{blue}{TODO: Only apparent observations are not enough.}
In Figure \ref{fig:interpretation-probe} we demonstrate the performance of layer-wise LR probes and cross-layer aggregation of each layer for both frozen and fine-tuned GPT2-XL models. This result shows that on the first layer, only features within the cumulative importance threshold are utilized hence accounting for a slight decrement in performance, and afterward STC consistently outperforms the layer-wise probing results. Specifically, during the first half of the layers, the aggregated method yields smooth rises in the curves above the layer-wise probes. After the layer-wise curves reach their peaks and start to retrace, the aggregated curves manage to maintain their performance and even achieve slight improvements till the final layer of the models.}


\rmv{This aggregation forms a composite representation $\bm{\Tilde{X}}_{\text{Agg},L_\text{temp}}$ and $\bm{\Tilde{A}}_{\text{Agg},L_\text{temp}}$, by concatenating the activations and hidden states of selected salient neurons from the previous layer-wise sparsification process:}

\rmv{
$g(\bm{\Tilde{X}}_{\text{Agg},L_\text{temp}}, f)$ and $g(\bm{\Tilde{A}}_{\text{Agg},L_\text{temp}}, f)$, which yields logistic predictors $\bm{\Hat{Y}}_{\text{Agg}, X,L\text{temp}}=\sigma(g(\bm{\Tilde{X}}_{\text{Agg},L_\text{temp}},f) \bm{\Hat{W}}_{X,L_\text{temp}}+\bm{\Hat{b}}_{X,L_\text{temp}})$ and $\bm{\Hat{Y}}_{\text{Agg}, A,L\text{temp}}=\sigma(g(\bm{\Tilde{A}}_{\text{Agg},L_\text{temp}},f) \bm{\Hat{W}}_{A,L_\text{temp}}+\bm{\Hat{b}}_{A,L_\text{temp}})$ for each $L_\text{temp}$, as our text classifiers. 

To summarize, we present the overall algorithm design of STC within \ref{linear-probing}, \ref{layer-wise-sparsification} and \ref{cross-layer-aggregation} as an end-to-end solution for leveraging the internal representations of LLMs for text classification tasks, as illustrated in Algorithm \ref{alg:stc}.


\begin{alignat*}{2}
\bm{\Hat{W}}_{X,L_\text{temp}},\bm{\Hat{b}}_{X,L_\text{temp}} &= \arg \min_{\bm{W},\bm{b}}||\bm{Y}-\sigma(g(\bm{\Tilde{X}}_{\text{Agg},L_\text{temp}},f)\bm{W}+\bm{b})||_1+\lambda||\bm{W}||_1, \qquad &&L_\text{temp}=0,\cdots, L \\
\bm{\Hat{W}}_{A,L_\text{temp}},\bm{\Hat{b}}_{A,L_\text{temp}} &= \arg \min_{\bm{W},\bm{b}}||\bm{Y}-\sigma(g(\bm{\Tilde{A}}_{\text{Agg},L_\text{temp}},f)\bm{W}+\bm{b})||_1+\lambda||\bm{W}||_1, \qquad &&L_\text{temp}=0, \cdots, L-1
\end{alignat*}
} 

\rmv{
\begin{algorithm}[tb]
\caption{Sparsify then Classify}
\label{alg:stc}
\begin{small}
\begin{algorithmic}
\STATE {\bfseries Input:}$\{g(\bm{\Tilde{A}}_l, f),\quad l\in\{0,\cdots,L_\text{temp}-1\}\}, \bm{Y}, \eta\in(0,1)$
\STATE {\bfseries Output:}$\bm{\Hat{Y}}_{\text{Agg}}=\sigma(g(\bm{\Tilde{A}}_{\text{Agg}},f) \bm{\Hat{W}}+\bm{\Hat{b}}), \Hat{l}_\text{Agg}$ 
\STATE Initialize $\bm{\Tilde{A}}_{\text{Agg}} \gets \varnothing$\; $\bm{\Hat{Y}}_{\text{Agg}} \gets \varnothing$\; $\Hat{l}_\text{Agg} \gets 0$\; $l \gets 0$\;
\WHILE{$l < L_\text{temp}$}
    %\tcc{Layer-wise LR Probing}
    \STATE$\bm{\Hat{W}},\bm{\Hat{b}} \gets \arg \min_{\bm{W},\bm{b}}||\bm{Y}-\sigma(g(\bm{\Tilde{A}}_l,f)\bm{W}+\bm{b})||_1+\lambda||\bm{W}||_1$\;
    %\tcc{Layer-wise Sparsification}
    \STATE$\bm{J} \gets$ index$(\bm{\Hat{W}})$\;
    \STATE$\bm{\Hat{W}}, \bm{J}\gets$ sort$(\bm{\Hat{W}}, \bm{J})$\;
    \STATE$\bm{S} \gets \varnothing$\; $\Sigma \gets 0$\; $k \gets 1$\;
    \WHILE{$\Sigma \leq \eta \cdot||\bm{\Hat{W}}||_2^2$}
        \STATE$\bm{S} \gets \bm{S}\cup\{\bm{J}_{k}\}$\;
        \STATE$\Sigma \gets \Sigma + (\bm{\Hat{W}}_{k})^2$\;
        \STATE$k \gets k+1$\;
    \ENDWHILE
\ENDWHILE
%\tcc{Cross-layer Aggregation}
\STATE$\bm{\Tilde{A}}_{\text{Agg}} \gets \bm{\Tilde{A}}_{\text{Agg}} \cup \{\bm{\Tilde{A}}_{l,i}\forall i\in\bm{S}\}$\;

\STATE$\bm{\Hat{W}},\bm{\Hat{b}} \gets \arg \min_{\bm{W},\bm{b}}||\bm{Y}-\sigma(g(\bm{\Tilde{A}}_{\text{Agg}},f)\bm{W}+\bm{b})||_1+\lambda||\bm{W}||_1$\;

\STATE$\bm{\Hat{Y}}=\sigma(g(\bm{\Tilde{A}}_{\text{Agg}},f) \bm{\Hat{W}}+\bm{\Hat{b}})$\;
\IF{$||\bm{Y}-\bm{\Hat{Y}}||_1 < ||\bm{Y}-\bm{\Hat{Y}}_\text{Agg}||_1$}
    \STATE$\bm{\Hat{Y}}_\text{Agg} \gets \bm{\Hat{Y}}$\;
    \STATE$\Hat{l}_\text{Agg} \gets l$\;
\ENDIF
\end{algorithmic}
\end{small}
\end{algorithm}
}

\rmv{
\begin{algorithm}[tb]
   \caption{Bubble Sort}
   \label{alg:example}
\begin{algorithmic}
   \STATE {\bfseries Input:} data $x_i$, size $m$
   \REPEAT
   \STATE Initialize $noChange = true$.
   \FOR{$i=1$ {\bfseries to} $m-1$}
   \IF{$x_i > x_{i+1}$}
   \STATE Swap $x_i$ and $x_{i+1}$
   \STATE $noChange = false$
   \ENDIF
   \ENDFOR
   \UNTIL{$noChange$ is $true$}
\end{algorithmic}
\end{algorithm}
}

\begin{table*}[t]
%\vspace*{-2cm}
\caption{Performance of LLM application in text classification for baselines and \emph{Sparsify-then-Classify}}
\label{tab:best_compare}
\centering
\small
\begin{tabular}{r@{\hspace{6pt}}l >{\centering}p{4.5em}@{\hspace{6pt}}>{\centering}p{5.5em}@{\hspace{6pt}} >{\centering}p{3.8em}@{\hspace{6pt}}>{\centering}p{3.8em} >{\centering}p{3.8em}@{\hspace{6pt}}>{\centering\arraybackslash}p{3.8em}}
    \toprule
    & & \multicolumn{2}{c}{\textbf{Baseline}} & \multicolumn{2}{c}{\textbf{Frozen + STC}} & \multicolumn{2}{c}{\textbf{Fine-tuned + STC}}\\
    \cmidrule(lr){3-4} \cmidrule(lr){5-6} \cmidrule(lr){7-8}
    \textbf{Dataset} & \textbf{Model} & \textbf{Embedding} & \textbf{Fine-tuning}\tablefootnote{For the model fine-tuning baseline, results without brackets are excerpted from the HuggingFace profiles of the corresponding fine-tuned models we used for STC, and results with brackets are measured in our own experiments due to the lack of reported data.} & \textbf{Probes} & \textbf{Agg.} & \textbf{Probes} & \textbf{Agg.} \\
    \midrule
    \multirow{10}{*}{\shortstack[r]{IMDb\\(acc.)}} 
    & DistilBERT & 86.95 & 92.80 & 88.94 & \textbf{89.49} & 92.76 & \textbf{92.88} \\ 
    & RoBERTa    & 89.67 & 95.52 & 92.20 & \textbf{93.38} & 95.52 & \textbf{95.68} \\
    & GPT2       & 85.46 & 93.94 & 90.02 & \textbf{91.94} & 93.98 & \textbf{93.99+} \\
    & GPT2-M     & 88.72 &(90.70)& 92.51 & \textbf{93.91} & 93.04 & \textbf{93.92} \\
    & GPT2-L     & 91.76 &(92.74)& 93.22 & \textbf{94.28} & 93.92 & \textbf{94.76} \\
    & GPT2-XL    & 91.86 &(93.11)& 94.59 & \textbf{94.92} & 94.50 & \textbf{95.12} \\
    & XLNet (SotA) & 86.42 & 95.70 & 93.08 & \textbf{93.15} & 95.72 & \textbf{95.72} \\
    & Flan-T5-Small    & 77.58 & \textemdash & 90.33 & \textbf{91.15} & \textemdash & \textemdash \\
    & Flan-T5-Base    & 79.66 & 93.32 & 93.82 & \textbf{94.15} & \textemdash & \textemdash \\
    & Flan-T5-Large    & 85.74 & \textemdash & 94.49 & \textbf{96.02} & \textemdash & \textemdash \\
    & Flan-T5-XL   & 90.31 & \textemdash & 95.95 & \textbf{96.13} & \textemdash & \textemdash \\
    \midrule        
    \multirow{10}{*}{\shortstack[r]{GLUE\\SST-2\\(val acc.)}} 
    & DistilBERT & 84.06 & \textbf{91.30} & 84.06 & \textbf{84.40} & 90.59 & 91.19 \\
    & RoBERTa    & 84.06 & 94.03 & 88.76 & \textbf{90.59} & 94.15 & \textbf{94.38} \\
    & GPT2       & 85.89 & 91.51 & 85.89 & \textbf{87.73} & 91.63 &  \textbf{92.32} \\
    & GPT2-M     & 84.63 & 91.98 & 86.58 & \textbf{90.25} & 92.09 & \textbf{92.32} \\
    & GPT2-L     & 90.14 & \textemdash & 90.94 & \textbf{91.97} & \textemdash & \textemdash \\
    & GPT2-XL    & 90.02 & \textemdash & 91.86 & \textbf{93.23} & \textemdash & \textemdash \\
    & Flan-T5-Small    & 75.00 & \textemdash & 87.27 & \textbf{88.99} & \textemdash & \textemdash \\
    & Flan-T5-Base    & 85.89 & 94.38 & 89.79 & \textbf{92.32} & \textemdash & \textemdash \\
    & Flan-T5-Large    & 77.41 & \textemdash & 93.46 & \textbf{94.84} & \textemdash & \textemdash \\
    & Flan-T5-XL   & 84.75 & \textemdash & 94.04 & \textbf{95.64} & \textemdash & \textemdash \\
    \midrule        
    \multirow{10}{*}{\shortstack[r]{EDOS\\Task A\\(Macro F1)}} 
    & DistilBERT & 65.09 & 78.74 & 71.16 & \textbf{75.79} & 80.44 & \textbf{81.12} \\
    & RoBERTa    & 68.81 & 80.48 & 70.84 & \textbf{73.50} & 80.32 & \textbf{80.88} \\
    & GPT2      & 68.57 & \textemdash & 72.53 & \textbf{76.08} & \textemdash & \textemdash \\
    & GPT2-M     & 71.17 & \textemdash & 72.57 & \textbf{75.74} & \textemdash & \textemdash \\
    & GPT2-L     & 72.05 & \textemdash & 73.44 & \textbf{76.33} & \textemdash & \textemdash \\
    & GPT2-XL    & 72.56 & \textemdash & 73.88 & \textbf{76.69} &\textemdash & \textemdash \\
    & Flan-T5-Small    & 59.62 & \textemdash & 67.88 & \textbf{74.51} & \textemdash & \textemdash \\
    & Flan-T5-Base    & 66.64 & \textemdash & 72.31 & \textbf{78.04} & \textemdash & \textemdash \\
    & Flan-T5-Large    & 69.58 & \textemdash & 74.38 & \textbf{79.00} & \textemdash & \textemdash \\
    & Flan-T5-XL   & 70.08 & \textemdash & 76.09 & \textbf{81.48} & \textemdash & \textemdash \\
    \bottomrule 
\end{tabular}
%\vspace*{-0.5cm}
\end{table*}

\rmv{, which consistently outperforms the model output, for arbitrary types of transformer-based language models.}

\rmv{
\paragraph{Conventional LLM Text Classification Baselines} In the realm of text classification, LLMs have been applied with different methodologies and focal areas. Traditional paradigms include the following three: sentence embedding method, model fine-tuning, and in-context learning. The sentence embedding approach, following \cite{mikolov2013efficient}, primarily utilizing encoder-focused LLMs, leverages the last layer's hidden states of single tokens, focusing on generating sentence-level embeddings for text classification without modifying model weights or prompt fine-tuning, as demonstrated in seminal works by \cite{le2014distributed}, \cite{devlin2018bert}, \cite{reimers2019sentence}, etc. In contrast, the model fine-tuning approach involves a comprehensive adaptation of the entire LLM structure, including model weights and classification heads, for task-specific adjustments, with research including \cite{howard2018universal}, \cite{sun2019fine} and \cite{yu2019improving} demonstrating the effectiveness. The in-context learning (ICL) approach, exemplified by a trend of generative models after GPT-3 (\cite{brown2020language}), adopts a decoder-focused structure and relies on prompt-based learning without altering model weights or using a separate classification head, offering a flexible and prompt-driven methodology. 

\paragraph{Interpreting Internal Representations} The internal representations have long been a canon perspective in interpreting the decision-making process of AI models. Classic models like word2vec \citep{mikolov2013efficient} initially illustrated the linearly interpretable semantic features found within the word embedding space. \cite{alain2016understanding} introduced the concept of linear \emph{probes} for deep convolutional networks. Subsequent works in LLMs have furthered our understanding of how they acquire task-specific knowledge, including studies on how FFN layers operate as key-value memories \cite{geva2020transformer}, the concept of knowledge neurons within transformer-based models \cite{dai2021knowledge}, and identification of internal units as task-specific experts based on their pattern of activations \cite{suau2020finding}. \cite{burns2022discovering} and \cite{gurnee2023language} have explored the encoding of spatial, temporal, and factual data within LLMs. Recent work by OpenAI including \cite{bills2023language} extends our understanding of LLMs by letting GPT4 to interpret the different levels of features captured by individual neurons in GPT2-XL. This collection of research has provided vast evidence of internal representations in LLMs being able to capture task-specific features.

\paragraph{Leveraging Internal Representations as Text Classifiers} Leveraging activations and hidden states of LLMs for text classification tasks has gained traction. Studies as early as \cite{radford2017learning} have shown the potential of utilizing individual neuron activations in LSTM to conduct sentiment classification. Research by \cite{durrani2020analyzing} and \cite{gurnee2023finding} provided further insights into hidden states being used for linguistic and factual representation in models like ELMo, BERT, and the Pythia family. Closely relevant research also includes \cite{wang2022finding} identifying specific neurons within RoBERTa that are responsible for particular skills over neuron activations, and empirically validating the potential of using the top-ranked task-specific neurons for classification with competitive performance. Moreover, \cite{durrani2022linguistic} and \cite{gurnee2023language} from the LLaMA2 family, demonstrated the effectiveness of leveraging these internal representations for more nuanced and specific text classification tasks. These works highlight the adaptability and robustness of LLMs in text classification by employing innovative techniques like sparse probing to unravel the complexities within the internal representations, and herald the potential for better text classifiers using neuron representations than LM head or classification head.
}

% In the existing literature of interpretability in transformer-based language models, it is important to note the \emph{linear representation hypothesis}, which posits that features within neural networks are represented linearly \citep{mikolov2013efficient, elhage2022softmax}. Meanwhile, linear probe \citep{alain2016understanding} is a prevalent tool to unravel the linear relationships between internal feature representations and target concepts or labels. Therefore, our investigation focuses on the technique of linear probing on each layer independently within LLM internal representations, which is widely adopted for interpretability and evaluating the quality of features in LLMs \citep{dalvi2019one, suau2020finding, wang2022finding, gurnee2023finding}.

% Given the pooled results of hidden states and FFN activations, we train logistic regressors (LR) with $\mathcal{L}^1$-regularization, also known as Lasso regularization, as the linear classifier probes, to predict the category which input texts belong to. Each layer of the LLMs is examined independently to understand the behavior and contribution of neurons at different depths. 

% \rmv{
% For LR probes, the objective is to predict the target $\bm{Y}\in\mathbb{R}^{B}$ from pooled hidden states $g(\bm{\Tilde{X}}_l,f) \in \mathbb{R}^{B\times D}$ or activations $g(\bm{\Tilde{A}}_l,f) \in \mathbb{R}^{B\times (kD)}$ for all $B$ sentences at a given layer $l$ of model. The optimization problem for fitting LR probes with $\mathcal{L}^1$-regularization is formulated as:
% \begin{alignat*}{2}
% \bm{\Hat{W}}_{X,l},\bm{\Hat{b}}_{X,l} &= \arg \min_{\bm{W},\bm{b}}||\bm{Y}-\sigma(g(\bm{\Tilde{X}}_l,f)\bm{W}+\bm{b})||_1+\lambda||\bm{W}||_1, \qquad&&l=0,\cdots, L \\
% \bm{\Hat{W}}_{A,l},\bm{\Hat{b}}_{A,l} &= \arg \min_{\bm{W},\bm{b}}||\bm{Y}-\sigma(g(\bm{\Tilde{A}}_l,f)\bm{W}+\bm{b})||_1+\lambda||\bm{W}||_1, \qquad&&l=0, \cdots, L-1
% \end{alignat*}
% where $\sigma(\cdot)$ denotes the logistic sigmoid function, and $\lambda \geq 0$ is the regularization parameter that controls the trade-off between the fidelity of the model to the training data and the complexity of the model's weights. The term $||\bm{W}||_1$ represents the $\mathcal{L}^1$-norm of the weight vector, which is the sum of the absolute values of the weights. The regularization term controlled by hyper-parameter $\lambda$, encourages sparsity in the weight vector, effectively performing feature selection by driving certain weights to zero. The regression yields a logistic predictor $\bm{\Hat{Y}}_X=\sigma(g(\bm{\Tilde{X}}_l,f)\bm{\Hat{W}}_{X,l}+\bm{\Hat{b}}_{X,l})$ and $\bm{\Hat{Y}}_A=\sigma(g(\bm{\Tilde{A}}_l,f)\bm{\Hat{W}}_{A,l}+\bm{\Hat{b}}_{A,l})$ of each layer for inference.
% }

%\subsection{Layer-wise Sparsification}
% \label{layer-wise-sparsification}
% One aspect of the $\mathcal{L}^1$-regularized LR probes is that the learned weights $\bm{\Hat{W}}$ can be interpreted as indicators of the importance of neurons at that layer for the specific task \citep{guyon2003introduction, ng2004feature}. In essence, LR probes provide a mechanism to identify task-specific salient neurons within the internal representations of LLMs. Weights with higher magnitudes suggest that the corresponding neurons play a more crucial role in making task-specific predictions. By the sparsity of $\mathcal{L}^1$-regularized LR weights \citep{tibshirani1996regression}, where weights have been inherently pushed towards zero with less important features often having weights exactly at zero, we derive an intuitive criterion for neuron selection. 

% \rmv{
% Here we consider the trained LR probes as sparsified salient feature indicators by investigating the magnitude of weights they learned. Given logistic predictor $\bm{\Hat{Y}}_X=\sigma(g(\bm{\Tilde{X}}_l,f)\bm{\Hat{W}}_{X,l}+\bm{\Hat{b}}_{X,l})$ and $\bm{\Hat{Y}}_A=\sigma(g(\bm{\Tilde{A}}_l,f)\bm{\Hat{W}}_{A,l}+\bm{\Hat{b}}_{A,l})$ for each layer $l=0,\cdots, L_\text{temp}$ as the LR probes we trained independently based on each layer's hidden states and activations by running the LLM up to layer $L_\text{temp}$, we focus on the logistic regression weights $\bm{\Hat{W}}_{X,l}\in\mathbb{R}^D$ and $\bm{\Hat{W}}_{A,l}\in\mathbb{R}^{(kD)}$.

% In this context, a measure that rewards larger weights is advantageous, as it aligns with the underlying assumption that a higher logistic regression weight correlates with stronger informativeness and a more significant contribution the corresponding input feature makes to the model's predictive capacity. Consequently, ranking neurons according to their absolute magnitude of weights in trained linear probes yields good feature selection results in LLMs \citep{bau2018identifying, dalvi2019one}. At the same time, selecting a large number of features, especially those that are not strongly predictive of the outcome, will dilute the effect of the predictive features and make it harder to identify the signal amidst the noise \citep{guyon2003introduction}. }


% To encourage better layer-wise sparsification, we introduce the squared $\mathcal{L}^2$-norm from the perspective of signal processing to being employed as a measure of the \emph{energy} exerted by the LR weights. Mathematically, the squared $\mathcal{L}^2$-norm of a weight vector effectively amplifies the impact of larger weights, thereby providing a unified scale that accentuates the more influential features in terms of their contribution to the model's predictions \citep{hastie2009elements}. On this foundation, a sparsification threshold $\eta$ is established. When the cumulative sum of weights for a set of neurons, whose weights are sorted in descending order in advance, exactly exceeds the $\eta$ quota of the total cumulative sum, we designate the given set of neurons as salient. 

% \rmv{This process, similar to the weight pruning techniques in neural networks \citep{lecun1989optimal} that adopts backward elimination of variables, can effectively filter out neurons with minimal impact.}

% \rmv{on the squared $\mathcal{L}^2$-norm $||\bm{\Hat{W}}_{X,l}||_2^2$ and $||\bm{\Hat{W}}_{A,l}||_2^2$, which is calculated by the sum of squared weights corresponding all input features within that layer, serving as a measure of the cumulative importance of different features' contributions to the layer's LR probe. By sorting all squared feature weights in descending order and calculating the cumulative sum across features, we can assess the collective importance of any given set of individual features.} 


% In this study, we focus on the internal representations widely involved in previous literature: hidden states $\bm{X}_l\in\mathbb{R}^{N\times D}$ \citep{durrani2020analyzing, burns2022discovering, gurnee2023language} and activations $\bm{A}_l\in \mathbb{R}^{N\times kD}$ of feed-forward network neurons \citep{bills2023language, gurnee2023finding} of each layer, where the dimension of hidden space within the FFN, i.e., the number of FFN neurons, is often set as a multiple of $D$. 

% \rmv{
% In Section \ref{preliminaries-internal} we have described how the last layer of hidden state records are condensed token-wise by the pooling function extracting the result on the specific position at a certain single token, which is purely based on the way the model is pretrained on the last layer of output, ignoring the large amount of potentially useful information inside the sentence and model. Previous studies \citep{bills2023language} have shown that the activations among tokens within the sentence input also hold meaningful position-specific patterns that vary across different layers of the model, intuitively suggesting more expressive representations to be utilized. 

% Hence in this study, we investigate the FFN activations and hidden states for all layers
% \begin{alignat*}{2}
% g(\bm{X}_l,f_\text{single}:\mathbb{R}^N\mapsto\mathbb{R})&: \mathbb{R}^{N\times D} \mapsto \mathbb{R}^D \qquad &&l=0,\cdots, L\\
% g(\bm{A}_l,f_\text{single}:\mathbb{R}^N\mapsto\mathbb{R})&: \mathbb{R}^{N\times A} \mapsto \mathbb{R}^{A} \qquad &&l=0,\cdots, L-1
% \end{alignat*}
% along with two more pooling methods, average pooling and max pooling, to additionally express more detailed information about how specific neurons are activated across tokens within a sentence. 
% }

% Traditional classification methods typically rely on outputs corresponding to single tokens, which not effectively encapsulate sentence-level information. This limitation is particularly relevant for internal representations, as a substantial portion of the model's architecture does not inherently aggregate information at the token level. To overcome this, we introduce two more pooling strategies—average pooling and max pooling—designed to map these variable-length internal representations into a fixed-size feature space. These strategies enable us to capture a more comprehensive statistical profile of neuron activations across different tokens within a sentence.  

